How to Find a Good Explanation for Clustering?

$k$-means and $k$-median clustering are powerful unsupervised machine learning techniques. However, due to complicated dependences on all the features, it is challenging to interpret the resulting cluster assignments. Moshkovitz, Dasgupta, Rashtchian, and Frost [ICML 2020] proposed an elegant model of explainable $k$-means and $k$-median clustering. In this model, a decision tree with $k$ leaves provides a straightforward characterization of the data set into clusters. We study two natural algorithmic questions about explainable clustering. (1) For a given clustering, how to find the "best explanation" by using a decision tree with $k$ leaves? (2) For a given set of points, how to find a decision tree with $k$ leaves minimizing the $k$-means/median objective of the resulting explainable clustering? To address the first question, we introduce a new model of explainable clustering. Our model, inspired by the notion of outliers in robust statistics, is the following. We are seeking a small number of points (outliers) whose removal makes the existing clustering well-explainable. For addressing the second question, we initiate the study of the model of Moshkovitz et al. from the perspective of multivariate complexity. Our rigorous algorithmic analysis sheds some light on the influence of parameters like the input size, dimension of the data, the number of outliers, the number of clusters, and the approximation ratio, on the computational complexity of explainable clustering.

==> otherwork.tex <==
 %!TEX root = neurips_2021.tex
\medskip\noindent\textbf{Related work.}  Recently, post-modeling explainable techniques have received critiques due to their lack of generality \cite{rudin2019stop}. We note that the explainable clustering model of Moshkovitz et al.\cite{MoshkovitzDRF20} falls in the scope of pre-modeling explainability while  \probClustExpl is in the scope of post-modeling explainability.
 Although there is a huge amount of work on explainability in the context of supervised learning, explainable unsupervised learning has received comparatively less attention. The most popular explainability model used in the context of clustering is based on decision trees \cite{BertsimasOW21,fraiman2013interpretable,geurts2007inferring,ghattas2017clustering,lipton2018mythos,MoshkovitzDRF20}. Most of these works are empirical in nature. As mentioned before, the work of Moshkovitz et al. \cite{MoshkovitzDRF20} is the first theoretical work on explainable clustering. Following this work, Laber and Murtinho \cite{laber2021price} proved dimension dependent bounds on the price of explainability, in particular, $O(d\log k)$ for $k$-median and $O(dk\log k)$ for $k$-means objectives. These bounds improve the bounds in \cite{MoshkovitzDRF20} in case the dimension is small. See the thesis by Cannone~\cite{connonethesis} for other models of explainable clustering. 


==> ourwork.tex <==
 %!TEX root = neurips_2021.tex

\medskip\noindent\textbf{Our results.} 
 Our work sheds some light on the   influence of  parameters like the input size $n$, dimension of the data $d$, the number of outliers $s$, the number of clusters $k$, and the approximation ratio $\varepsilon$,    on the computational complexity of explainable clustering.

Our first result, Theorem~\ref{thm:exp-w} establishes that
\probEMeanClust and \probEMedClust are NP-hard. Actually, our reduction shows that the problems cannot be solved in  $f(k)\cdot n^{o(k)}$ time for a computable function $f(\cdot)$ unless Exponential Time Hypothesis (ETH) fails.  This shows that the running time $(4nd)^{k+\Oh(1)}$ of the  trivial brute-force algorithm (Observation~\ref{obs:naive}) is asymptotically optimal.  We also obtain algorithms solving  \probEMeanClust and \probEMedClust in time 
$n^{2d}\cdot (dn)^{\Oh(1)}$, which is polynomial for  fixed $d$. 

It is possible to obtain better algorithms with dependence on $k$ and $d$ if we relax the requirements on the quality of the solution. 
 More precisely, we define  \probFMeanExpl  as follows. For a collection of $n$ points $\bfX\subseteq \mathbb{R}^d$ and a positive real constant $\varepsilon<1$, we seek whether we can
   identify at most $\varepsilon n$ outliers, such that the cost of explainable $k$-means of the remaining points does not exceed the optimal cost of an explainable $k$-means clustering of the original data set. The problem  \probFMedExpl is defined similarly. 
 For   \probFMeanExpl and \probFMedExpl we give algorithms whose running time $(\frac{8dk}{\epsilon})^k\cdot n^{\Oh(1)}$ has a significantly better dependence on $d$ and $k$. 

We also show that providing a simple explanation to a given $k$-clustering is a challenging computational task. We prove that 
 \probClustExpl, the problem to decide whether an obtained $k$-clustering admits a good explanation after deleting at most $s$ points, could not be approximated within a factor of $F(s)$ in time $f(s) (nd)^{o(s)}$, for any functions $F$ and $f$, unless ETH fails.  On the other hand, we give a polynomial-time $(k-1)$-approximation algorithm for the optimization version of \probClustExpl. 
When it comes to exact algorithms, we give an algorithm solving  \probClustExpl in time 
$2^{2\min\{s,k\}}\cdot n^{2d}\cdot (dn)^{\Oh(1)}$. We also provide an efficient preprocessing procedure (polynomial kernelization in the language of parameterized complexity \cite{FominLSZ19}) that reduces an instance of   \probClustExpl  to an equivalent instance with at most $r=2(s+1)dk$ points in $\mathbb{R}^d$ with integer coordinates within the range  $\{1,\ldots, r\}$.


